A Versatile, Sound Tool for Simplifying Definitions

We present a tool, simplify-defun, that transforms the definition of a given function into a simplified definition of a new function, providing a proof checked by ACL2 that the old and new functions are equivalent. When appropriate it also generates termination and guard proofs for the new function. We explain how the tool is engineered so that these proofs will succeed. Examples illustrate its utility, in particular for program transformation in synthesis and verification.

==> eptcsdata.tex <==
\providecommand{\firstpage}{61}
\providecommand{\publicationstatus}{Warren Hunt Jr.\ and Anna Slobodova (Eds.):\\
ACL2 Theorem Prover and its Applications\\
EPTCS 249, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.249.5}{10.4204/EPTCS.249.5}}

